A topological characterisation of the Kashiwara-Vergne groups

In 2017 Bar-Natan and the first author showed that solutions to the Kashiwara--Vergne equations are in bijection with certain knot invariants: homomorphic expansions of welded foams. Welded foams are a class of knotted tubes in $\mathbb{R}^4$, which can be finitely presented algebraically as a circuit algebra, or, equivalently, a wheeled prop. In this paper we describe the Kashiwara-Vergne groups $\mathsf{KV}$ and $\mathsf{KRV}$ -- the symmetry groups of Kashiwara-Vergne solutions -- as automorphisms of the completed circuit algebras of welded foams, and their associated graded circuit algebra of arrow diagrams, respectively. Finally, we provide a description of the graded Grothendieck-Teichm\"uller group $\mathsf{GRT}_1$ as automorphisms of arrow diagrams.

==> relationship_to_grt.tex <==
\section{The image of $\mathsf{GRT}_1$ in $\krv$}\label{sec:krvgrt}
The Grothendieck--Teichm\"uller groups $\gt$ and $\grt_1$, defined by Drinfeld in \cite{Drin90}, are known to act freely and transitively on the set of all Drinfeld associators. It was shown by Bar-Natan \cite[Proposition 4.5, Proposition 4.8]{BNGT} that $\grt_1$ is isomorphic to the automorphisms of parenthesised chord diagrams; and later understood that this same result could be concisely presented using operads in \cite{tamarkin1998proof} and \cite[Theorem 10.3.6]{FresseVol1}. In their paper \cite{AT12},  Alekseev and Torossian establish a close relationship between the graded Grothendieck--Teichm\"uller group and the group $\krv$,  conjecturing that $\krv\cong \mathbb{Q}t\times \grt_1$ (\cite[Section 4; Remark 9.14]{AT12}).  In this section we demonstrate how, using the relationship between $\grt_1$ and $\krv$ established by Alekseev and Torossian, we can describe $\grt_1$ as certain automorphisms of arrow diagrams.


\subsection{$\grt_1$ as automorphisms of an operad} %Solutions to the KV conjecture are about automorphisms of free Lie algebras while Drinfeld associators are automorphisms of the Lie algebra of infinitesimal braids. 
We briefly recall the description of the Grothendieck-Teichm\"{u}ller group $\grt_1$ as automorphisms of the operad of parenthesised chord diagrams. The interested reader can find a more in-depth description in \cite{BNGT}, \cite{FresseVol1} or \cite{merkGT}.  The Lie algebra of \emph{infinitesimal braids} on $n$ strands, $\mathfrak{t}_n$, $n\geq 2$, is the quotient of the free Lie algebra $\lie_{\frac{n(n-1)}{2}}$ generated by the symbols $\{t_{i,j} = t_{j,i}\}_{1\leq i< j\leq n}$ subject to the relations \[ [t_{i,j} , t_{k,l}] = 0  \quad \text{and} \quad[t_{i,j} , t_{i,k} + t_{k,j}] = 0 \] whenever $i,j,k,l$ are distinct. 

The completed universal enveloping algebra, $\widehat{U}(\mathfrak{t}_n)$, can be viewed as a category of \emph{chord diagrams} on $n$ strands, $\mathsf{CD}(n)$. This category has one object and is enriched in (completed, filtered, coassociative) coalgebras (e.g. \cite[Section 6.4]{merkGT}). Morphisms of $\mathsf{CD}(n)$ are depicted as chord diagrams on $n$ vertical strands, where $t_{i,j}$ is represented by a chord between strands $i$ and $j$. Composition of morphisms is depicted by ``stacking'' the chord diagrams. The collection of categories $\mathsf{CD}:=\{\mathsf{CD}(n)\}$, $n\geq 2$, forms an operad in which operadic composition is defined by a cabling operation (Figure~\ref{operad composition CD}).  Every operation in $\mathsf{CD}$ can be generated by operadic and categorical compositions using a single generator $t_{1,2}:=\chord\in\mathsf{CD}(2)$. 
\begin{figure}[h]

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.5,xscale=.5]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da20962765479610124] 
\draw [line width=1.5]    (31,60) -- (30,200) ;
%Straight Lines [id:da3079804645913835] 
\draw [line width=1.5]    (71,60) -- (70,200) ;
%Straight Lines [id:da4697382453519505] 
\draw [line width=1.5]    (110,60) -- (110,200) ;
%Straight Lines [id:da4084834826750323] 
\draw [line width=1.5]    (199,60) -- (199,200) ;
%Straight Lines [id:da6617415536428318] 
\draw [line width=1.5]    (240,60) -- (240,200) ;
%Straight Lines [id:da29559295987878165] 
\draw     (29,120) -- (69,120) ;
%Straight Lines [id:da5261549233082581] 
\draw    (30,140) -- (109,140) ;
%Straight Lines [id:da31243773394519103] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]    (200,121) -- (238.18,121) ;
%Straight Lines [id:da8649031572076119] 
\draw [line width=1.5]    (371,60) -- (370,200) ;
%Straight Lines [id:da528306244897487] 
\draw [line width=1.5]    (411,60) -- (410,200) ;
%Straight Lines [id:da00017329642341368245] 
\draw [line width=1.5]    (449,60) -- (449,200) ;
%Straight Lines [id:da1447841875932958] 
\draw   (371,120) -- (411,120) ;
%Straight Lines [id:da4694323847339429] 
\draw [line width=1.5]    (538,60) -- (537,200) ;
%Straight Lines [id:da8139016588083937] 
\draw [line width=1.5]    (578,60) -- (577,200) ;
%Straight Lines [id:da0806306292336294] 
\draw [line width=1.5]    (616,60) -- (616,200) ;
%Straight Lines [id:da6957118726199151] 
\draw    (537,122) -- (617,122) ;
%Straight Lines [id:da37125593194230166] 
\draw     (538,142) -- (653,142) ;
%Straight Lines [id:da2725563061227515] 
\draw [line width=1.5]    (491,60) -- (491,200) ;
%Straight Lines [id:da47009591936307593] 
\draw [line width=1.5]    (652,60) -- (652,200) ;
%Straight Lines [id:da16890241592803523] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]    (413,110) -- (449,110) ;
%Straight Lines [id:da06951848053968257] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]    (579,102) -- (617,102) ;
%Straight Lines [id:da15329054559094046] 
\draw (371,141) -- (491,141) ;

% Text Node
\draw (142,120) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$\circ _{2}$};
% Text Node
\draw (500,120) node [anchor=north west][inner sep=0.75pt]    {$+$};
% Text Node
\draw (295,120) node [anchor=north west][inner sep=0.75pt]    {$=$};


\end{tikzpicture}
\caption{An example of composition in the operad $\mathsf{CD}$.}\label{operad composition CD}
\end{figure}


\medskip 

%The group $\grt_1$ is isomorphic to automorphisms of the operad of \emph{parenthesised chord diagrams}. 
The category of \emph{parenthesised chord diagrams}, $\mathsf{PaCD}(n)$, is obtained by formally replacing the object of the category $\mathsf{CD}(n)$ with the set of parenthesised words of length $n$ with distinct letters. Let $M(n)$ denote the subset of parenthesised monomials in $\{1, ..., n\}$ where each element of the set occurs exactly once.\footnote{Equivalently, $M(n)$ may denote the set of binary rooted trees, leaves labelled from the set $\{1, ..., n\}$, where each element of the set occurs exactly once.} For example, $(12)(3(45))$ is an element in $M(5)$. The symmetric group $\calS_n$ acts on the right of $M(n)$ by permuting the elements of the set $\{1, ..., n\}$ and there is an obvious map $u : M(n)\rightarrow \ast$ which collapses every monomial to a point (e.g. \cite[Section 10.3.1]{FresseVol1}). 



The category $\mathsf{PaCD}(n)$ is the pullback of the category $\mathsf{CD}(n)$ along the map $u$.  In other words, the set of objects of $\mathsf{PaCD}(n)$ is $M(n)$. Morphisms between any two $p_i,p_j\in M(n)$ are defined as $$\Hom_{\mathsf{PaCD}(n)}(p_i,p_j) := \Hom_{\mathsf{CD}(n)}(\ast,\ast) = \widehat{U}(\mathfrak{t}_n).$$ Categorical composition makes $\PaCD(n)$ into a Hopf groupoid\footnote{Technically, in the \cite{FresseVol1} presentation, the morphisms of $\PaCD(n)$ are only the \emph{group-like} elements of $ \widehat{U}(\mathfrak{t}_n)$.}  \cite[Section 10.3.2]{FresseVol1}.

\medskip 

The collection of all parenthesised chord diagrams, $\mathsf{PaCD}:=\{\mathsf{PaCD}(n)\}_{n\geq 2}$, forms an operad in Hopf groupoids. At the level of objects, operadic composition is given by replacing letters by monomials.\footnote{Alternatively, operadic composition is given by grafting binary trees.} For example, we have the following composition $(1(34))(25)\circ_4 (13)2 = (1(3((46)5)))(27)$. The operadic composition of morphisms is the operadic composition of $\mathsf{CD}$. See \cite{BNGT} or Chapter 10.3.1~\cite{FresseVol1} for full details. 

Every operation in the operad $\mathsf{PaCD}$ can be written as a combination of operadic and categorical compositions of three generators: \[\virtualcrossing\in \Hom_{\mathsf{PaCD}(2)}((12), (21)), \quad \chord\in  \Hom_{\mathsf{PaCD}(2)}((12), (12))\quad \text{and} \quad \Associator\in \Hom_{\mathsf{PaCD}(3)}((12)3,1(23)).\] These generating morphisms are considered up to the \emph{pentagon} and  two \emph{hexagon} relations (notation explained below): 
\begin{equation}\label{PaCD pentagon}  d_1\Associator \cdot d_3 \Associator= d_4 \Associator \cdot d_2 \Associator \cdot d_0 \Associator \end{equation} 
\begin{equation}\label{PaCD hexagon} d_1\virtualcrossing =  \Associator \cdot d_0\virtualcrossing \cdot ((23) (\Associator)^{-1})\cdot (23)d_3\virtualcrossing\cdot (321)\Associator\end{equation} 
\begin{equation}\label{PaCD hexagon2} d_1(\virtualcrossing)^{-1} =  \Associator \cdot d_0(\virtualcrossing)^{-1} \cdot ((23) (\Associator)^{-1})\cdot (23)d_3 (\virtualcrossing)^{-1}\cdot (321)\Associator\end{equation}
Here, the operation $d_0$ adds an "empty" strand to the left of the chord diagram, and $d_{n+1}$ adds an empty strand to the right. For $1\leq i \leq n$, the operation $d_i$ {\em doubles} the $i$th strand of a chord diagram (similar to the {\em unzip} operation of arrow diagrams). This is described on the generators $t_{j,k}$ as follows (see \cite[Definition 2.9]{BNGT}):\[ d_i(t_{j,k})=\begin{cases} t_{j+1,k+1} \ \text{if} \  i < j < k \\ t_{j,k+1} + t_{j+1,k+1} \ \text{if} \ i=j<k \\ t_{j,k+1} \ \text{if} \ j < i < k \\ t_{j,k} + t_{j,k+1} \ \text{if} \ j < i = k \\ t_{j,k} \ \text{if} \ j < k < i .\end{cases}\]  

\begin{definition}\cite[Section 4.2]{AT12}
The graded Grothendieck--Teichm\"uller group $\grt_1$ is the exponentiation of the Lie algebra $\mathfrak{grt}_1$ spanned by derivations $\psi=(0,\psi)\in\tder_2$ which satisfy the following equations: 
\begin{equation}\label{inversion}
\psi(x,y)=-\psi(y,x),
\end{equation} 
\begin{equation}\label{hexagon} 
\psi(x,y)+\psi(y,z) +\psi(z,x) =0 \quad \text{ whenever } x+y+z=0
\end{equation} 
\begin{equation}\label{pentagon}  
\psi(t_{1,2},t_{2,34})+\psi(t_{12,3},t_{3,4}) =\psi(t_{2,3},t_{3,4})+\psi(t_{1,23},t_{23,4})+\psi(t_{1,2},t_{2,3}).
\end{equation} 
 \end{definition} 
In equation \eqref{pentagon}, $t_{i,j}\in\mathfrak{t}_4$ and the notation $t_{ij,k}$ is shorthand for $t_{i,k}+t_{j,k}$. Similarly, $t_{i,jk}=t_{i,j}+t_{i,k}$.  
\medskip 

Let $\Aut(\mathsf{PaCD})$ denote the group of automorphisms of the operad $\mathsf{PaCD}$ which fix objects and the elements $\virtualcrossing\in \Hom_{\mathsf{PaCD}(2)}((12), (21))$ and $\chord\in  \Hom_{\mathsf{PaCD}(2)}((12), (12))$. The following theorem can be found in \cite[Proposition 4.5, Proposition 4.8]{BNGT} or \cite[Theorem 10.3.6]{FresseVol1}. See also \cite{tamarkin1998proof} or \cite[Section 6.7]{merkGT}. 
 

\begin{theorem}\label{thm: GRT is Aut} 
There is an isomorphism of groups $\Aut(\mathsf{PaCD})\cong\grt_1$. 
\end{theorem} 


We do not reproduce the proof of Theorem~\ref{thm: GRT is Aut} in this paper, but we will use the following key points.  Since every element of $\PaCD$ can be written via operadic and categorical compositions of $\chord$, $\virtualcrossing$ and $\Associator$, it follows that any automorphism  $G\in\Aut(\PaCD)$ is uniquely determined by its value $G(\Associator)= \Psi(t_{1,2}, t_{2,3})$, where $\Psi=e^\psi$ is an element of $\widehat{U}(\lie_2)$. Since $G$ is an automorphism of $\PaCD$, $G$ respects the pentagon \eqref{PaCD pentagon} and hexagon \eqref{PaCD hexagon}, \eqref{PaCD hexagon2} relations, which means that $\Psi=e^{\psi}$ satisfies equations \eqref{inversion}, \eqref{hexagon} and \eqref{pentagon} and is therefore in $\grt_1$. 




%\begin{remark} 
%Our brief sketch of the proof of Theorem~\ref{thm: GRT is Aut} looks tantalizingly similar to the proof of Theorem~\ref{thm: aut(A)=KRV}\ihnote{Did I reference the right theorem here?}. As such, it is tempting to try to compare $\grt_1$ and $\krv$ by ``mapping'' the operad of parenthesised chords into the circuit algebra of arrow diagrams. Unfortunately, operads and circuit algebras are not compatible algebraic structures and one cannot expect any kind of homomorphism $\mathsf{PaCD}\rightarrow \arrows$. 
%\end{remark} 
\subsection{$\grt_1$ as automorphisms of arrow diagrams} 
 Alekseev and Torossian \cite[Theorem 4.6]{AT12}) provide an injective Lie algebra homomorphism $\varrho: \mathfrak{grt}_1 \rightarrow \mathfrak{krv}_2$ given by
 \[ \psi \mapsto (\psi(-x-y,x), \psi(-x-y,y)). \] Combining this result with those of Theorem~\ref{thm: aut(A)=KRV} and the now classical Theorem~\ref{thm: GRT is Aut}, we have following commutative diagram of groups: \[\begin{tikzcd}
\Aut(\PaCD) \arrow[d, "\cong", swap]\arrow[r, dotted, "\tilde{\varrho}"] & \Aut_v(\arrows) \arrow[d, "\cong"] \\
\grt_1 \arrow[r, "\exp(\varrho)"] & \krv
 \end{tikzcd}\] In order to describe the graded Grothendieck-Teichm\"uller group $\grt_1$ as automorphisms of arrow diagrams, we first describe the image of $\tilde{\varrho}$ in $\Aut_{v}(\arrows).$  
 

\subsubsection{The relationship between $\PaCD$ and $\arrows$}  The algebraic structures of $\PaCD$ and $\arrows$ are different: operads do not embed directly into circuit algebras. Nonetheless, we can describe the image of the underlying collection of Hopf groupoids $\bigcup_{n}\PaCD(n)$ inside the circuit algebra $\arrows$.  

For any $n\geq 2$, there is an inclusion of Lie algebras $\mathfrak{t}_n\hookrightarrow \tder_n$, where $\mathfrak{t}_n$ is isomorphic to a Lie subalgebra of $\tder_n$ spanned by tangential derivations of the form $t^{i,j}=(0,\ldots, x_j,\ldots, x_i,\ldots 0)$,  with non-vanishing components $x_i$ at the $j$th place and $x_j$ at the $i$th place \cite[Proposition 3.11]{AT12}.  The inclusion $\mathfrak{t}_n\hookrightarrow \tder_n$ extends to a Hopf algebra homomorphism \[\begin{tikzcd}\Hom_{\mathsf{CD}(n)}(\ast,\ast):=\widehat{U}(\mathfrak{t}_n)\arrow[r] & \widehat{U}(\tder_n\oplus \mathfrak{a}_n \ltimes \cyc_n)  \arrow[r, "\cong"', "\Upsilon^{-1}"] &  \arrows(\uparrow_n).\end{tikzcd}\] 

 

\begin{lemma}\label{Hopf CD lemma}
For each $n\geq 2$ there exists an inclusion of Hopf algebras \[\begin{tikzcd}\Hom_{\mathsf{CD}(n)}(\ast,\ast)\arrow[r, "\varepsilon"]& \arrows(\uparrow_n).\end{tikzcd}\]
\end{lemma} 

\begin{proof}
We start by defining a linear map $\begin{tikzcd}\Hom_{\mathsf{CD}(n)}(\ast,\ast):=\widehat{U}(\mathfrak{t}_n)\arrow[r, "\varepsilon"]& \arrows(\uparrow_n).\end{tikzcd}$ The generating element $t_{i,j}$ in $\mathfrak{t}_{n}$ is represented as a chord diagram in $\widehat{U}(\mathfrak{t}_n)$ which has a single chord connecting the $i$th vertical strand to the $j$th vertical strand (e.g. $t_{1,2}=\chord$). We set $\varepsilon(t_{i,j})$ to be the sum of two arrow diagrams:  the first a single arrow going from strand $i$ to $j$ and the second a single arrow going from $j$ to $i$. In other words, we send the chord diagram $t_{i,j}$ to the arrow diagram $\Upsilon^{-1}(t^{i,j})$. In particular, $\varepsilon(t_{1,2})=\varepsilon(\chord)=\rarrow + \larrow$. By \cite[Proposition 3.11]{AT12}, this map is well-defined as the $t^{i,j}$s satisfy the relations of $\mathfrak{t}_n$. 

The coproduct on $\mathsf{CD}(n)$ is defined on generators as $\Delta_{\mathsf{CD}}(t_{i,j})=t_{i,j}\otimes 1 + 1\otimes t_{i,j}$. It is now straightforward to check that $\varepsilon(\Delta_{\mathsf{CD}}(t_{i,j}))=\Delta_{\arrows}(\varepsilon(t_{i,j}))$, where the latter is defined in Definition~\ref{def: coprod}. Similarly, the product commutes with $\varepsilon$ since the categorical composition of $\mathsf{CD}(n)$ corresponds to circuit algebra composition given by the wiring diagram $\WD_s$ (Figure~\ref{WD for stacking}) which stacks arrow diagrams on $n$ strands. 
%In other words, the following diagram
%\[\begin{tikzcd} \Hom_{\mathsf{CD}(n)}(\ast,\ast)\times Hom_{\mathsf{CD}(n)}(\ast,\ast) \arrow[r] \arrow[d, swap, "\varepsilon\times\varepsilon"]& Hom_{\mathsf{CD}(n)}(\ast,\ast) \arrow[d, "\varepsilon"]\\
%\arrows(\uparrow_n)\times \arrows(\uparrow_n) \arrow[r, "\WD_{s}"] & \arrows(\uparrow_n) \end{tikzcd}\] commutes and the lemma follows. 
\end{proof} 


Next, we extend Lemma~\ref{Hopf CD lemma} to an inclusion of Hopf groupoids $\begin{tikzcd}\PaCD(n)\arrow[r, "\varepsilon"]& \arrows\end{tikzcd}$ by working ``one skeleton at a time''. For any two objects $p_1,p_2$ in $\PaCD(n)$, the empty chord diagram in $\Hom_{\PaCD(n)}(p_1,p_2)$ has an underlying permutation $p_2^{-1}p_1\in\mathcal{S}_n$ (here $p_1$, $p_2 \in M(2)$ are considered as permutations interpreted in the one-line notation). As we saw in Example~\ref{ex: w-tangle skeleton}, there is a corresponding skeleton in $\calS$. We have already implicitly used this idea when we write $\virtualcrossing$ for the empty chord diagram in $\Hom_{\PaCD(2)}((12),(21))$ which has underlying permutation $(21)\in\calS_2$.  The empty chord diagram in $\Hom_{\PaCD(n)}(p_1,p_2)$ carries the additional structure of the parenthesisations $p_1$ and $p_2$ which we can encode by ``closing up'' the skeleton permutation $p_2^{-1}p_1$ with binary trees at the bottom and top\footnote{As a general convention we draw diagrams "bottom to top". That is, $p_1$ is shown at the bottom and morphisms travel up to $p_2$.}
 according to the parenthesisations $p_1$ and $p_2$. We will denote this skeleton element by $c_{p_1p_2}$ in $\arrows$. For example, the closure of $\Associator\in\Hom_{\PaCD(3)}((12)3, 1(23))$ is the skeleton element $\bubble\in \arrows$ depicted in Figure~\ref{def: bubble}. 

\begin{figure}[h]
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.5,xscale= .8]


%Shape: Ellipse [id:dp35228824509455015] 
\draw   (458,154.5) .. controls (458,120.53) and (476.13,93) .. (498.5,93) .. controls (520.87,93) and (539,120.53) .. (539,154.5) .. controls (539,188.47) and (520.87,216) .. (498.5,216) .. controls (476.13,216) and (458,188.47) .. (458,154.5) -- cycle ;
%Straight Lines [id:da2797990977977364] 
\draw    (466,191) -- (530,117) ;
%Straight Lines [id:da7554179628606673] 
\draw    (498.5,216) -- (499,244) ;
%Straight Lines [id:da2981137171240188] 
\draw    (498.5,93) -- (498,61) ;
%Straight Lines [id:da052771676828520686] 
\draw    (99,99.81) -- (98,234.81) ;
%Straight Lines [id:da21680543217879278] 
\draw    (162,101.81) -- (161,236.81) ;
%Straight Lines [id:da7497021927332164] 
\draw [->]   (212,170) -- (417,170) ;
%Curve Lines [id:da3787919199400831] 
\draw    (107,235) .. controls (114,196) and (147,151) .. (150,102) ;

% Text Node
\draw (35,235) node [anchor=north west][inner sep=0.75pt]    {$p_{1} \ =$};
% Text Node
\draw (35,90) node [anchor=north west][inner sep=0.75pt]    {$p_{2} \ =$};
% Text Node
\draw (282,145) node [anchor=north west][inner sep=0.75pt]    {$c_{p_{1}p_{2}}$};
% Text Node
\draw (85,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {(};
% Text Node
\draw (138,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {(};
% Text Node
\draw (80,226) node [anchor=north west][inner sep=0.75pt]   [align=left] {(};
% Text Node
\draw (113,226) node [anchor=north west][inner sep=0.75pt]   [align=left] {)};
% Text Node
\draw (165,226) node [anchor=north west][inner sep=0.75pt]   [align=left] {)};
% Text Node
\draw (165,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {)};
% Text Node
\draw (170,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {)};
% Text Node
\draw (85,226) node [anchor=north west][inner sep=0.75pt]   [align=left] {(};


\end{tikzpicture}
\caption{The closure of $\Associator$ in $\arrows$. }\label{def: bubble} 
\end{figure} 


We define the map
\begin{equation} \begin{tikzcd} \Hom_{\PaCD(n)}(p_1,p_2)\arrow[r, "\varepsilon"] &\arrows(c_{p_1p_2})\end{tikzcd}\label{linear map PaCD to A}\tag{$\star$}\end{equation} 
as the composition of the old  $\varepsilon$ (as in Lemma~\ref{Hopf CD lemma}) applied to the underlying morphism of $\mathsf{CD}(n)$, followed by the skeleton closure. Letting $p_i,p_j$ run over all objects in $\PaCD(n)$, we have the following theorem. 

\begin{theorem}\label{inclusion of Hopf groupoids} The categorical composition of $\PaCD(n)$ can be realised using the operations in $\bigcup_{c_{p_ip_j}} \arrows(c_{p_ip_j})$, and this elevates $\varepsilon$ to an inclusion of Hopf groupoids
\[\begin{tikzcd} \PaCD(n)\arrow[r, "\varepsilon"]& \bigcup_{c_{p_ip_j}} \arrows(c_{p_ip_j}).\end{tikzcd}\] 
\end{theorem}

We split the proof of this theorem into three lemmas: first, we show that the categorical composition of $\PaCD(n)$ can be realised in $\bigcup_{c_{p_ip_j}} \arrows(c_{p_ip_j})$ to make $\varepsilon$ multiplicative. Then we show that $\varepsilon$ is well-defined, that is, it respects the pentagon and hexagon relations.

\begin{lemma}\label{lem:emultiplicative}
The categorical composition of $\PaCD(n)$ can be realised using the operations of $\bigcup_{c_{p_ip_j}} \arrows(c_{p_ip_j})$ to make $\varepsilon$ multiplicative.
\end{lemma}

\begin{proof} We need to define a composition operation on $\bigcup_{c_{p_ip_j}} \arrows(c_{p_ip_j})$ in a way that makes the maps \eqref{linear map PaCD to A} compatible with categorical composition in $\PaCD(n)$. This is summarised in the following commutative diagram, for any $p_1,p_2,p_3\in\PaCD(n)$:
\begin{equation}\label{stacking}
\begin{tikzcd} \Hom_{\PaCD(n)}(p_1,p_2)\otimes \Hom_{\PaCD(n)}(p_2,p_3)\arrow[d, "\circ", swap]\arrow[r, "\varepsilon\times \varepsilon"]& \arrows(c_{p_1p_2}) \otimes \arrows (c_{p_2p_3}) \arrow[d, "u^{n-1}\WD_s"] \\
\Hom_{\PaCD(n)}(p_1,p_3) \arrow[r, "\varepsilon"]& \arrows(c_{p_1p_3}) 
\end{tikzcd}
\end{equation}
In the diagram \eqref{stacking}, the left vertical map is categorical composition in $\PaCD$ and the right vertical map is given by first "stacking" (a circuit algebra operation using a wiring diagram as in Figure~\ref{WD for stacking}), and then applying the unzip operation $n-1$ times to eliminate the vertices in the middle, as in Figure~\ref{fig:ClosureComp}.  
\end{proof} 


Recall that every element of the operad $\PaCD$ can be obtained by iterated categorical and operadic compositions of the morphisms $\chord$, $\Associator$ and $\virtualcrossing$. Moreover, these generating morphisms satisfy the pentagon and hexagon relations \eqref{PaCD pentagon}, \eqref{PaCD hexagon}, and \eqref{PaCD hexagon2}. The operadic composition of $\PaCD$ is not preserved by $\varepsilon$ (that is, not realised by circuit algebra operations, unzips and orientation switches). However, operadic composition is not required for stating the pentagon and hexagon relations. This, and the multiplicativity of $\varepsilon$ helps show below that these relations are preserved by 

\begin{equation}\label{eq:ue}\tag{$\star\star$}
\begin{tikzcd}
\bigcup\limits_{n\geq 2}\PaCD(n) \arrow[r, "\cup\varepsilon"]& \arrows.
\end{tikzcd}
\end{equation}

\begin{figure}
\[
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp6678928487453082] 
\draw   (293,90.53) .. controls (293,64.55) and (307.76,43.48) .. (325.97,43.48) .. controls (344.17,43.48) and (358.93,64.55) .. (358.93,90.53) .. controls (358.93,116.51) and (344.17,137.58) .. (325.97,137.58) .. controls (307.76,137.58) and (293,116.51) .. (293,90.53) -- cycle ;
%Straight Lines [id:da9710513874813407] 
\draw    (299.51,118.45) -- (351.6,61.84) ;
%Straight Lines [id:da10153416338262256] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (325.97,137.58) -- (326.37,159) ;
%Straight Lines [id:da27882035357518253] 
\draw    (325.97,43.48) -- (325.56,19) ;
%Shape: Ellipse [id:dp7876499403457988] 
\draw   (294.29,223.49) .. controls (294.29,198.24) and (308.77,177.78) .. (326.64,177.78) .. controls (344.51,177.78) and (359,198.24) .. (359,223.49) .. controls (359,248.73) and (344.51,269.19) .. (326.64,269.19) .. controls (308.77,269.19) and (294.29,248.73) .. (294.29,223.49) -- cycle ;
%Straight Lines [id:da9562062593358984] 
\draw    (304.08,257.98) -- (355.21,202.99) ;
%Straight Lines [id:da05604686737123066] 
\draw    (326.64,269.19) -- (327.04,290) ;
%Straight Lines [id:da23475048250132824] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (326.64,177.78) -- (326.24,154) ;
%Shape: Arc [id:dp8115446555911434] 
\draw  [draw opacity=0] (353.25,114.21) .. controls (349.08,111.46) and (346,101.9) .. (346,90.53) .. controls (346,78.68) and (349.34,68.79) .. (353.79,66.53) -- (355.72,90.53) -- cycle ; \draw   (353.25,114.21) .. controls (349.08,111.46) and (346,101.9) .. (346,90.53) .. controls (346,78.68) and (349.34,68.79) .. (353.79,66.53) ;
%Shape: Arc [id:dp28564073923636224] 
\draw  [draw opacity=0] (300.81,193.73) .. controls (305.43,197.33) and (308.13,206.24) .. (307.14,216.36) .. controls (306.07,227.24) and (301.1,236.03) .. (295.35,238.08) -- (294.47,215.29) -- cycle ; \draw   (300.81,193.73) .. controls (305.43,197.33) and (308.13,206.24) .. (307.14,216.36) .. controls (306.07,227.24) and (301.1,236.03) .. (295.35,238.08) ;
%Shape: Ellipse [id:dp1496673205857768] 
\draw   (462,154.09) .. controls (462,110.1) and (484.83,74.44) .. (513,74.44) .. controls (541.17,74.44) and (564,110.1) .. (564,154.09) .. controls (564,198.08) and (541.17,233.74) .. (513,233.74) .. controls (484.83,233.74) and (462,198.08) .. (462,154.09) -- cycle ;
%Straight Lines [id:da7111048015880623] 
\draw    (469,193) -- (541,88) ;
%Straight Lines [id:da3214850137427565] 
\draw    (513,233.74) -- (513.63,270) ;
%Straight Lines [id:da20639941867697176] 
\draw    (513,74.44) -- (512.37,33) ;
%Straight Lines [id:da7445610575414237] 
\draw    (484,220) -- (558,115) ;
%Straight Lines [id:da5188584238163465] 
\draw [->]   (367,153) -- (436,153) ;
%Straight Lines [id:da04902927669840573] 
\draw    (62,40) -- (62,140) ;
%Straight Lines [id:da5553639383761588] 
\draw    (82,40) -- (82,140) ;
%Straight Lines [id:da5998369373851833] 
\draw    (102,40) -- (102,140) ;
%Straight Lines [id:da7728835570847521] 
\draw    (122,40) -- (122,140) ;
%Straight Lines [id:da9580904091230229] 
\draw    (62,180) -- (62,285) ;
%Straight Lines [id:da5425491150187467] 
\draw    (82,180) -- (82,285) ;
%Straight Lines [id:da9104113088426318] 
\draw    (102,180) -- (102,285) ;
%Straight Lines [id:da37929141657837806] 
\draw    (123,180) -- (123,285) ;
%Straight Lines [id:da9839127613735819] 
\draw [->]   (162,151) -- (252,151) ;
%Shape: Rectangle [id:dp8582201218448027] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (56,218) -- (126,218) -- (126,237) -- (56,237) -- cycle ;
%Shape: Rectangle [id:dp19316050097281945] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (56,78) -- (126,78) -- (126,97) -- (56,97) -- cycle ;
%Shape: Rectangle [id:dp6506083187645129] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (293,80) -- (358,80) -- (358,96) -- (293,96) -- cycle ;
%Shape: Rectangle [id:dp08848937627677356] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (295,214) -- (359,214) -- (359,230) -- (295,230) -- cycle ;
%Shape: Rectangle [id:dp622174723374378] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (463,165) -- (563,165) -- (563,186) -- (463,186) -- cycle ;
%Shape: Rectangle [id:dp758476101129921] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (463,125) -- (563,125) -- (563,145) -- (463,145) -- cycle ;

% Text Node
\draw (395,135) node [anchor=north west][inner sep=0.75pt]    {$u^{3}$};
% Text Node
\draw (207,135) node [anchor=north west][inner sep=0.75pt]    {$c$};
% Text Node
\draw (50,175) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$( ($};
% Text Node
\draw (94,175) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (94,133) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (50,133) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (45,278) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$((($};
% Text Node
\draw (83,175) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (124,175) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (124,133) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (83,133) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (128,133) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (53,133) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (128,175) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
%\draw (53,175) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (125,278) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (83,278) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
\draw (103,278) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)$};
% Text Node
%\draw (53,280) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
%\draw (46,280) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (124,34) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$)))$};
% Text Node
\draw (92,34) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (73,34) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};
% Text Node
\draw (53,34) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$($};


\end{tikzpicture}
\]
\caption{Closure and composition of chord diagrams.}\label{fig:ClosureComp}
\end{figure}

\begin{lemma}\label{lem: pentagon in arrows}
The map  \eqref{eq:ue} respects the pentagon relation. That is, the $\varepsilon$-images of the two sides of the pentagon relation coincide in $\arrows$. 
\end{lemma}

\begin{proof} 
Recall that the pentagon equation \eqref{PaCD pentagon} in $\PaCD$ is 
\begin{equation*} 
d_1\Associator \cdot d_3 \Associator = d_4 \Associator \cdot d_2 \Associator \cdot d_0 \Associator.
\end{equation*}
We apply the closure operation to each of the $d_i\Associator$ to get the corresponding skeleton element $d_i\bubble$, $0\leq i\leq 4$.\footnote{The notation $d_i\bubble$ is only convenient shorthand for the closure of $d_i\Associator$, as the strand doubling operation $d_i$ does not translate directly to a circuit algebra or auxiliary operation, though it can be described in diagrammatic terms as a version of strand doubling.}
We then multiply these elements in $\arrows$ using the operation $u^{n-1}\WD_s$, as in the diagram \eqref{stacking}.
In particular, the image of $d_1\Associator \cdot d_3 \Associator $ in $\arrows$ is the composite of the two ``bubbles'' pictured on the left in Figure~\ref{LHS pentagon}. Completely unzipping the interior of this composite results in the third ``bubble'' on the left in Figure~\ref{LHS pentagon}. Similarly, the element $d_4 \Associator \cdot d_2 \Associator \cdot d_0 \Associator$ corresponds to the stacking of bubbles depicted on the right of Figure~\ref{RHS pentagon}. Completely unzipping the interior results in the third bubble on the right in Figure~\ref{RHS pentagon}. It follows that  \begin{equation}\label{pentagon arrows} d_1\bubble \cdot d_3 \bubble   =d_4 \bubble \cdot d_2 \bubble \cdot d_0 \bubble \end{equation} holds in $\arrows$ as both sides of the equation represent the same skeleton element. 
\end{proof}

\begin{figure}

\begin{subfigure}{0.3\textwidth}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.5,xscale=.5]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp9705212490788192] 
\draw   (58,84.34) .. controls (58,58.36) and (72.76,37.29) .. (90.97,37.29) .. controls (109.17,37.29) and (123.93,58.36) .. (123.93,84.34) .. controls (123.93,110.33) and (109.17,131.39) .. (90.97,131.39) .. controls (72.76,131.39) and (58,110.33) .. (58,84.34) -- cycle ;
%Straight Lines [id:da19834077184252819] 
\draw    (64.51,112.27) -- (116.6,55.65) ;
%Straight Lines [id:da36392284483828463] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (90.97,131.39) -- (91.37,152.81) ;
%Straight Lines [id:da1426934041177692] 
\draw    (90.97,37.29) -- (90.56,12.81) ;
%Shape: Ellipse [id:dp9151944948886398] 
\draw   (59.29,217.3) .. controls (59.29,192.06) and (73.77,171.59) .. (91.64,171.59) .. controls (109.51,171.59) and (124,192.06) .. (124,217.3) .. controls (124,242.54) and (109.51,263) .. (91.64,263) .. controls (73.77,263) and (59.29,242.54) .. (59.29,217.3) -- cycle ;
%Straight Lines [id:da0816670594122283] 
\draw    (69.08,251.8) -- (120.21,196.8) ;
%Straight Lines [id:da3102373140503272] 
\draw    (91.64,263) -- (92.04,283.81) ;
%Straight Lines [id:da1941525242794564] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (91.64,171.59) -- (91.24,147.81) ;
%Shape: Arc [id:dp8050668179722553] 
\draw  [draw opacity=0] (118.25,108.03) .. controls (114.08,105.28) and (111,95.71) .. (111,84.34) .. controls (111,72.49) and (114.34,62.61) .. (118.79,60.35) -- (120.72,84.34) -- cycle ; \draw   (118.25,108.03) .. controls (114.08,105.28) and (111,95.71) .. (111,84.34) .. controls (111,72.49) and (114.34,62.61) .. (118.79,60.35) ;
%Shape: Arc [id:dp26344899359820473] 
\draw  [draw opacity=0] (65.81,187.55) .. controls (70.43,191.14) and (73.13,200.05) .. (72.14,210.18) .. controls (71.07,221.06) and (66.1,229.84) .. (60.35,231.9) -- (59.47,209.11) -- cycle ; \draw   (65.81,187.55) .. controls (70.43,191.14) and (73.13,200.05) .. (72.14,210.18) .. controls (71.07,221.06) and (66.1,229.84) .. (60.35,231.9) ;
%Shape: Ellipse [id:dp26329224176773625] 
\draw   (225,150.9) .. controls (225,106.91) and (247.83,71.26) .. (276,71.26) .. controls (304.17,71.26) and (327,106.91) .. (327,150.9) .. controls (327,194.89) and (304.17,230.55) .. (276,230.55) .. controls (247.83,230.55) and (225,194.89) .. (225,150.9) -- cycle ;
%Straight Lines [id:da6561152874504911] 
\draw    (226,139.81) -- (304,84.81) ;
%Straight Lines [id:da7980718252921649] 
\draw    (276,230.55) -- (276.63,266.81) ;
%Straight Lines [id:da09069504828669617] 
\draw    (276,71.26) -- (275.37,29.81) ;
%Straight Lines [id:da28533486638169325] 
\draw    (247,216.81) -- (326,160.81) ;
%Shape: Arc [id:dp8074971199929004] 
\draw  [draw opacity=0] (225,150.9) .. controls (231.14,153.15) and (236.7,164) .. (238.16,177.58) .. controls (239.04,185.76) and (238.26,193.33) .. (236.3,198.86) -- (225.01,179.17) -- cycle ; \draw   (225,150.9) .. controls (231.14,153.15) and (236.7,164) .. (238.16,177.58) .. controls (239.04,185.76) and (238.26,193.33) .. (236.3,198.86) ;
%Shape: Arc [id:dp966977723753057] 
\draw  [draw opacity=0] (327,150.9) .. controls (318.53,146.41) and (311.81,130.77) .. (311.02,111.92) .. controls (310.75,105.53) and (311.19,99.45) .. (312.21,94) -- (330.64,111.1) -- cycle ; \draw   (327,150.9) .. controls (318.53,146.41) and (311.81,130.77) .. (311.02,111.92) .. controls (310.75,105.53) and (311.19,99.45) .. (312.21,94) ;
%Shape: Ellipse [id:dp8871247153647709] 
\draw   (442,147.9) .. controls (442,103.91) and (464.83,68.26) .. (493,68.26) .. controls (521.17,68.26) and (544,103.91) .. (544,147.9) .. controls (544,191.89) and (521.17,227.55) .. (493,227.55) .. controls (464.83,227.55) and (442,191.89) .. (442,147.9) -- cycle ;
%Straight Lines [id:da8205039619918193] 
\draw    (449,186.81) -- (521,81.81) ;
%Straight Lines [id:da4473972601613777] 
\draw    (493,227.55) -- (493.63,263.81) ;
%Straight Lines [id:da9638197140562822] 
\draw    (493,68.26) -- (492.37,26.81) ;
%Straight Lines [id:da813967951082121] 
\draw    (464,213.81) -- (538,108.81) ;
%Straight Lines [id:da8721692967011881] 
\draw [->]   (129,150) -- (198,150) ;
%\draw [shift={(200,150.81)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da534322488979473] 
\draw[->]    (347,150) -- (416,150) ;
%\draw [shift={(418,146.81)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (156,132) node [anchor=north west][inner sep=0.75pt]    {$u$};
% Text Node
\draw (375,120) node [anchor=north west][inner sep=0.75pt]    {$u^{2}$};
\end{tikzpicture}
\caption{The left hand side of the pentagon equation.}\label{LHS pentagon}
\end{subfigure} 
\hfill
\begin{subfigure}{0.3\textwidth}
\begin{tikzpicture}[x=0.75pt,y=0.5pt,yscale=-.75,xscale=.5]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp5059034172230277] 
\draw   (102.33,53.16) .. controls (102.33,34.04) and (112.68,18.54) .. (125.45,18.54) .. controls (138.22,18.54) and (148.57,34.04) .. (148.57,53.16) .. controls (148.57,72.27) and (138.22,87.77) .. (125.45,87.77) .. controls (112.68,87.77) and (102.33,72.27) .. (102.33,53.16) -- cycle ;
%Straight Lines [id:da6394447016338984] 
\draw    (107.18,73.98) -- (143.72,32.33) ;
%Straight Lines [id:da4317130954731442] 
\draw    (125.45,87.77) -- (125.45,106.06) ;
%Straight Lines [id:da5931553149237019] 
\draw    (125.74,18.82) -- (125.45,0.81) ;
%Curve Lines [id:da2151752310701901] 
\draw    (125.45,99.87) .. controls (74.21,99.87) and (75.21,7) .. (126.02,7) ;
%Shape: Ellipse [id:dp8552915656410194] 
\draw   (102.5,244.5) .. controls (102.5,223.43) and (112.84,206.35) .. (125.6,206.35) .. controls (138.36,206.35) and (148.71,223.43) .. (148.71,244.5) .. controls (148.71,265.57) and (138.36,282.65) .. (125.6,282.65) .. controls (112.84,282.65) and (102.5,265.57) .. (102.5,244.5) -- cycle ;
%Straight Lines [id:da8636027024794362] 
\draw    (107.35,267.45) -- (143.86,221.55) ;
%Straight Lines [id:da0879839735838005] 
\draw    (125.6,282.65) -- (125.6,302.81) ;
%Curve Lines [id:da5932701717063198] 
\draw    (125.6,292.73) .. controls (172.38,292.27) and (175.8,196.74) .. (125.75,196.74) ;
%Shape: Ellipse [id:dp7179568794802019] 
\draw   (100.84,152.87) .. controls (100.84,132.78) and (112.07,116.5) .. (125.92,116.5) .. controls (139.77,116.5) and (151,132.78) .. (151,152.87) .. controls (151,172.96) and (139.77,189.25) .. (125.92,189.25) .. controls (112.07,189.25) and (100.84,172.96) .. (100.84,152.87) -- cycle ;
%Straight Lines [id:da8841334643015969] 
\draw    (105.8,174.46) -- (145.43,130.69) ;
%Straight Lines [id:da4881189404748414] 
\draw    (125.92,189.25) -- (126.23,205.81) ;
%Straight Lines [id:da5266607974479384] 
\draw    (125.92,116.5) -- (125.61,97.57) ;
%Shape: Arc [id:dp8379248799826199] 
\draw  [draw opacity=0] (109.52,169.1) .. controls (108.26,163.92) and (110.55,156.05) .. (115.92,148.77) .. controls (123.05,139.1) and (133.01,133.98) .. (138.66,136.91) -- (125.9,155.48) -- cycle ; \draw   (109.52,169.1) .. controls (108.26,163.92) and (110.55,156.05) .. (115.92,148.77) .. controls (123.05,139.1) and (133.01,133.98) .. (138.66,136.91) ;
%Shape: Ellipse [id:dp8765483234673694] 
\draw   (310,151.53) .. controls (310,106.95) and (333.06,70.81) .. (361.5,70.81) .. controls (389.94,70.81) and (413,106.95) .. (413,151.53) .. controls (413,196.11) and (389.94,232.25) .. (361.5,232.25) .. controls (333.06,232.25) and (310,196.11) .. (310,151.53) -- cycle ;
%Straight Lines [id:da3870476884749692] 
\draw    (313,177.81) -- (388,84.81) ;
%Straight Lines [id:da2671453579394938] 
\draw    (361.5,232.25) -- (362.14,269) ;
%Straight Lines [id:da0699224963312649] 
\draw    (361.5,70.81) -- (360.86,28.81) ;
%Straight Lines [id:da655861818750936] 
\draw    (338,223.81) -- (410,125.81) ;
%Straight Lines [id:da15082009820947717] 
\draw[->]    (179,160) -- (297,160) ;
%\draw [shift={(299,162.81)}, rotate = 181.43] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (230,130) node [anchor=north west][inner sep=0.75pt]    {$u^{6}$};
\end{tikzpicture}
\caption{The right hand side of the pentagon equation.}\label{RHS pentagon}
\end{subfigure}
\caption{The two sides of the pentagon equation in $\arrows$.}
\end{figure} 


\begin{lemma}\label{lem: hexagon in arrows}
The map  \eqref{eq:ue} respects the hexagon relations. That is, the $\varepsilon$-images of the two sides of each hexagon relation coincide in $\arrows$. 
\end{lemma}


\begin{proof} 
Recall that the first hexagon relation \eqref{PaCD hexagon} in $\PaCD$ is 
\begin{equation*} \label{hexagon PaCD} 
d_1\virtualcrossing = \Associator \cdot d_0\virtualcrossing \cdot ((23) \Associator^{-1})\cdot (23)d_3\virtualcrossing\cdot (321)\Associator. 
\end{equation*} 
The element $\virtualcrossing\in\Hom_{\PaCD(2)}((12),(21))$ is the empty chord diagram on the transposition map; $\varepsilon$ maps this to the skeleton element $\twist\in A$. As before, we write $d_i\bubble$ or $d_j\twist$ for the skeleton closures of the morphisms $d_i\Associator$ and $d_j\virtualcrossing$ in $\PaCD$. One can then check, after fully unzipping the composite in Figure~\ref{hexagon pic} that the equation
 \begin{equation}\label{hexagon arrows} d_1\twist = \bubble \cdot d_0\twist \cdot ((23) \bubble^{-1})\cdot (23)d_3\twist \cdot (321)\bubble\end{equation} holds in $\arrows$. The second hexagon equation is similar. 
  \end{proof} 
 
 \begin{figure}[h]
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-.75,xscale=.75]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Ellipse [id:dp09441225382015006] 
\draw   (88.31,185.38) .. controls (61.16,184.2) and (39.83,169.67) .. (40.66,152.93) .. controls (41.49,136.19) and (64.17,123.58) .. (91.32,124.76) .. controls (118.47,125.94) and (139.81,140.47) .. (138.98,157.21) .. controls (138.15,173.95) and (115.46,186.56) .. (88.31,185.38) -- cycle ;
%Straight Lines [id:da000084073192904488] 
\draw    (40.66,152.93) -- (15.06,152.19) ;
%Shape: Free Drawing [id:dp532913675539645] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75] [line join = round][line cap = round] (42.37,163.88) .. controls (42.37,163.88) and (42.37,163.88) .. (42.37,163.88) ;
%Shape: Arc [id:dp1068643263259268] 
\draw  [draw opacity=0] (172.08,172.34) .. controls (167.26,167.02) and (164.46,160.73) .. (164.45,153.97) .. controls (164.4,134.79) and (186.78,119.18) .. (214.44,119.1) .. controls (242.09,119.02) and (264.55,134.51) .. (264.6,153.69) .. controls (264.61,159.52) and (262.55,165.02) .. (258.91,169.85) -- (214.52,153.83) -- cycle ; \draw   (172.08,172.34) .. controls (167.26,167.02) and (164.46,160.73) .. (164.45,153.97) .. controls (164.4,134.79) and (186.78,119.18) .. (214.44,119.1) .. controls (242.09,119.02) and (264.55,134.51) .. (264.6,153.69) .. controls (264.61,159.52) and (262.55,165.02) .. (258.91,169.85) ;
%Curve Lines [id:da2445426306345585] 
\draw    (172.59,172.9) .. controls (168.95,107.9) and (264.16,251.11) .. (258.5,170.4) ;
%Curve Lines [id:da029563620453509243] 
\draw    (172.59,172.9) .. controls (172.83,234.66) and (253.92,118.43) .. (258.5,170.4) ;
%Straight Lines [id:da7234651958469929] 
\draw    (265,153.81) -- (293.18,153.54) ;
%Straight Lines [id:da4348674935965473] 
\draw    (138.04,154.38) -- (164.46,154.36) ;
%Straight Lines [id:da7671000629489272] 
\draw    (59.23,130.86) -- (131.67,172.26) ;
%Shape: Ellipse [id:dp809608693128976] 
\draw   (340.49,187.24) .. controls (313.57,186.01) and (292.39,170.92) .. (293.18,153.54) .. controls (293.98,136.16) and (316.45,123.07) .. (343.37,124.3) .. controls (370.29,125.53) and (391.47,140.62) .. (390.67,158) .. controls (389.88,175.38) and (367.41,188.47) .. (340.49,187.24) -- cycle ;
%Straight Lines [id:da8943774105666804] 
\draw    (391,152.81) -- (415,152.81) ;
%Shape: Free Drawing [id:dp6337621433939373] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75] [line join = round][line cap = round] (294.89,164.91) .. controls (294.89,164.91) and (294.89,164.91) .. (294.89,164.91) ;
%Straight Lines [id:da11543676853523388] 
\draw    (298.68,168.97) -- (383.36,140.93) ;
%Shape: Arc [id:dp7217983106860808] 
\draw  [draw opacity=0] (505.92,135.98) .. controls (511.03,140.58) and (514.03,146.1) .. (514.06,152.05) .. controls (514.15,168.28) and (492.17,181.56) .. (464.96,181.71) .. controls (437.76,181.86) and (415.63,168.83) .. (415.54,152.6) .. controls (415.5,146.99) and (418.11,141.73) .. (422.65,137.25) -- (464.8,152.32) -- cycle ; \draw   (505.92,135.98) .. controls (511.03,140.58) and (514.03,146.1) .. (514.06,152.05) .. controls (514.15,168.28) and (492.17,181.56) .. (464.96,181.71) .. controls (437.76,181.86) and (415.63,168.83) .. (415.54,152.6) .. controls (415.5,146.99) and (418.11,141.73) .. (422.65,137.25) ;
%Curve Lines [id:da1781861739466345] 
\draw    (422.27,137.63) .. controls (423.63,85.96) and (508.12,191.88) .. (507.15,137.15) ;
%Curve Lines [id:da8356716544063166] 
\draw    (422.27,137.63) .. controls (420.38,193.12) and (503.67,82.54) .. (507.15,137.15) ;
%Straight Lines [id:da7798456779695218] 
\draw    (513.28,150.19) -- (532.52,150.08) ;
%Shape: Ellipse [id:dp1291765988059842] 
\draw   (579.02,180.85) .. controls (554.55,180.63) and (534.53,166.03) .. (534.29,148.24) .. controls (534.05,130.46) and (553.69,116.22) .. (578.15,116.45) .. controls (602.61,116.68) and (622.64,131.28) .. (622.88,149.06) .. controls (623.12,166.85) and (603.48,181.08) .. (579.02,180.85) -- cycle ;
%Straight Lines [id:da1772841086979473] 
\draw    (654,148.81) -- (622.88,149.06) ;
%Shape: Free Drawing [id:dp24996977471990578] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75] [line join = round][line cap = round] (534.14,158.65) .. controls (534.14,158.65) and (534.14,158.65) .. (534.14,158.65) ;
%Straight Lines [id:da9395562295179093] 
\draw    (547.09,125.19) -- (620,159.81) ;

\end{tikzpicture}
\caption{The right hand side of the image of the hexagon relation.
}\label{hexagon pic}
\end{figure}

{\em Proof of Theorem \ref{inclusion of Hopf groupoids}.} By Lemmas~\ref{lem: pentagon in arrows}~and~\ref{lem: hexagon in arrows}, $\varepsilon$ is well-defined. By definition, every $\Hom_{\PaCD(n)}(p_1, p_2)$ is a (completed, filtered coassocaitive) coalgebra so $\varepsilon$ is a map of (complete filtered, coassociative) coalgebras. Finally, by Lemma~\ref{lem:emultiplicative}, $\varepsilon$ is multiplicative.
\qed



\subsubsection{The image of $\grt_1$ in $\Aut_v(\arrows)$}
Recall that the Alekseev--Torossian map of Lie algebras $\varrho:\mathfrak{grt}_1\rightarrow \mathfrak{krv}_2$ induces a group homomorphism $\tilde{\varrho}$:

\begin{equation}\label{eq:rho}
\begin{tikzcd}
\Aut(\PaCD) \arrow[d, "\cong", swap]\arrow[r, dotted, "\tilde{\varrho}"] & \Aut_v(\arrows) \arrow[d, "\cong"] \\
\grt_1 \arrow[r, hookrightarrow, "\exp(\varrho)"] & \krv. 
 \end{tikzcd}
 \end{equation}
 
 The fact that $\tilde{\varrho}$ is a group homomorphism is automatic since $\tilde{\varrho}$ is a composite of group homomorphisms. Moreover, $\tilde{\varrho}$ is injective because $\varrho$ is injective. The image of $\Aut(\PaCD)$ in $\Aut_{v}(\arrows)$ is a subgroup of $\krv$ isomorphic to $\grt_1$. In Theorem~\ref{thm: GRT as Aut(A)} we give a direct description of $\grt_1$ as automorphisms of arrow diagrams whose value on $\bubble$ satisfies an additional condition. We start with two useful lemmas.

 
 \begin{lemma}\label{lem:bub}
 	For any $G_1, G_2 \in \Aut_{v}(\arrows)$, if $G_1(\bubble)=G_2(\bubble)$ then $G_1=G_2$.
 \end{lemma}  

\begin{proof} 
By Theorem \ref{thm: aut(A)=KRV}, an automorphism $G\in \Aut_v(\arrows)$ is determined by $G(\vertex)=N$. In particular, $\Upsilon(N)=e^we^n$, and $w$ is uniquely determined by $n$, so $G$ is determined by $n$.

For $i=1,2$, set $\Upsilon(G_i(\vertex))=e^{w_i}e^{n_i}$, and it is enough to prove that $n_1=n_2$. Since the $G_i$ are circuit algebra maps, we have
$$\Upsilon(G_i(\bubble))=\Upsilon((G_i(\vertex)^{12,3})^{-1}(G_i(\vertex)^{1,2})^{-1} G_i(\vertex)^{2,3}G_i(\vertex)^{1,23}).$$
The $\TAut_3$ (``tree'') component of this expression is:
$$(e^{-n_i})^{12,3}(e^{-n_i})^{1,2}) (e^{n_i})^{2,3}(e^{n_i})^{1,23} \in \TAut_3. $$     
Then, expanding the $\TAut_3$ component of $G_1(\bubble)G_2(\bubble)^{-1}=1$ degree by degree, using the above equation, we obtain that $n_1=n_2$, which implies the result.
\end{proof}

Recall that for $x\in \arrows(\uparrow_n)$ we denote $x^*=A_1A_2...A_n(x)$, where $A_i$ is the adjoint (direction switch) operation on strand $i$. The following fact from \cite{BND:WKO2} helps prove equalities between elements in $\arrows(\uparrow_n)$:
 
 \begin{lemma}\label{lem:TreeLemma}
 \cite[Lemma 4.16]{BND:WKO2}
 Two group-like elements $a$ and $b$ in $\arrows(\uparrow_n)$ are equal if and only if their ``tree components'' -- that is, their projections to $\exp(\tder_n \oplus \mathfrak{a}_n)$ -- are equal, and in addition $aa^*=bb^*$.  
 \end{lemma}

\begin{theorem}\label{thm: GRT as Aut(A)}
	The (isomorphic) image of $\grt_1$ in $\Aut_v(\arrows)$ is the subgroup $$\EB=\{\tilde{G} \in \Aut_v(\arrows)~:~\tilde{G}(\bubble)=\varepsilon(G(\Associator)) \text{ for some (unique) }G\in\Aut(\PaCD)\}.$$
\end{theorem}

\begin{proof} By the diagram \eqref{eq:rho}, the isomorphic image of $\grt_1$ in $\Aut_v(A)$ is $\tilde{\varrho}(\Aut(\PaCD))$. Therefore, we need to show that $\tilde{\varrho}(\Aut(\PaCD))=\EB$.
	
First, for an element $G \in \Aut(\PaCD)$, we show that $\tilde{G}:=\tilde{\varrho}(G) \in \EB$.
In the proof of Theorem~\ref{thm: GRT is Aut}, the isomorphism $\Aut(\PaCD)\cong \grt_1$ comes from the identification of $G(\Associator)=\Psi(t_{1,2},t_{2,3})$ where $\Psi=e^{\psi}$ for some $\psi\in\mathfrak{grt}_1$.  Applying $\exp(\varrho)$, we get an element $\exp(\varrho(\psi)):=\alpha \in \krv$. By Proposition 9.12 of \cite{AT12}, we have\footnote{Note that there is an inversion compared to \cite{AT12} as we follow the notation of \cite{ATE10}.}
\begin{equation}\label{eq:apsi}  \Psi(t^{1,2},t^{2,3})=\alpha^{12,3}\alpha^{1,2}(\alpha^{2,3})^{-1}(\alpha^{1,23})^{-1}\end{equation}
Recall that the element $\alpha \in \krv$ uniquely determines the corresponding Duflo series $s$. By Theorem~\ref{thm: aut(A)=KRV}, $\tilde{G}=\Theta^{-1}(\alpha)\in\Aut_v(\arrows)$ is given by
\[ 
\tilde{G}(\vertex):=\Upsilon^{-1}((\mathcal{J}(\alpha^{-1}))^{-\frac{1}{2}}\alpha^{-1}) \quad \text{and}\quad \tilde{G}(\upcap):=e^{-\kappa^{-1}(s)/2}.
\] 

Since $\tilde{G}$ is an automorphism of circuit algebras, we have (explained in more detail below):
\begin{equation}\label{eq:Gtilde}
\tilde{G}(\bubble)=(\tilde{G}(\vertex)^{12,3})^{-1}(\tilde{G}(\vertex)^{1,2})^{-1} \tilde{G}(\vertex)^{2,3}\tilde{G}(\vertex)^{1,23}.
\end{equation}
Here the cosimplicial notation on $\tilde{G}(\vertex)$ is the same as in Section~\ref{sec: cosimplicial structure}, keeping in mind that $\tilde{G}(\vertex)\in \arrows(\uparrow_2)$ by Lemma \ref{lemma: VI}. For example, $(\tilde{G}(\vertex)^{12,3})^{-1}$ is the value of the bottom vertex in $\bubble$. It is inverted as it is a vertex of the opposite orientation, see \cite[Proof of Theorem 4.9]{BND:WKO2}. A priori, this value is an arrow diagram on the top two strands of the bottom vertex. However, by the VI relation it can be ``pushed up'' to the middle three strands of the skeleton $\bubble$, this effectively doubles the first strand, hence the superscript ``$12,3$''.

Denote by $a$ the right hand side of Equation~\eqref{eq:Gtilde}, and by $b$  the $\Upsilon^{-1}$ value of the right hand side of equation \eqref{eq:apsi}. We use Lemma~\ref{lem:TreeLemma} to show that $a=b$. Observe that the tree components of $a$ and $b$ are the same (by definition of $\tilde{G}$). Furthermore, $aa^*=1$ by the \eqref{U'} equation. On the other hand, $bb^*=1$, as follows. The isomorphism $\Upsilon^{-1}$ maps $t^{i,j}$ to a sums of two horizontal arrows, and hence $(\Upsilon^{-1}(t^{ij}))^*= - \Upsilon^{-1}(t^{i,j})$. The group-like property $\Psi=e^{\psi}$ then implies that $\Upsilon^{-1}(\Psi(t^{1,2},t^{2,3}))\left(\Upsilon^{-1}(\Psi(t^{1,2},t^{2,3}))\right)^*=bb^*=1$. Therefore, $a=b$. In other words, this means that the ``wheel components'' of the vertex values in Equation~\eqref{eq:Gtilde} all cancel.

Applying $\Upsilon^{-1}$ to Equation \ref{eq:apsi}, note that $\Upsilon^{-1}\Psi(t^{1,2},t^{2,3})=\varepsilon(G(\Associator))$ by the definition of the map $\varepsilon$. Therefore, 
$\tilde{G}(\bubble)=\varepsilon(G(\Associator)),$ so $\tilde{G}\in \EB$.

Conversely, assume $\tilde{G}\in \EB$; we show that $\tilde{G}$ is in the image of $\tilde{\varrho}$. 
The statement $\tilde{G}\in \EB$ means that $\tilde{G} \in \Aut_v(\arrows)$ and $\tilde{G}(\bubble)=\varepsilon(G(\Associator))$ for some $G\in\Aut(\PaCD)$. 

Such a $G$ is unique, because $\varepsilon$ is injective and the value $G(\Associator)$ determines $G$. We will show that $\tilde{G}=\tilde{\varrho}(G)$, so $\tilde{G} \in \tilde{\varrho}(\Aut(\PaCD))$.
By the construction above, we know that $\tilde{\varrho}(G) \in \Aut_v(\arrows)$ satisfies $\tilde{\varrho}(G)(\bubble)=\varepsilon(G(\Associator))$. Therefore,
$$\tilde{\varrho}(G)(\bubble)=\tilde{G}(\bubble).$$
Applying Lemma \ref{lem:bub}, we get $\tilde{G}=\tilde{\varrho}(G)$.
\end{proof} 


